Resummed inclusive cross-section in ADD model at N$^3$LL+NNLO

We present three loop soft-plus-virtual (SV) corrections to the spin-2 production at the Large Hadron Collider (LHC). For this calculation, we make use of the recently computed quark and gluon three loop form factors for the spin-2 production, the universal soft-collinear coefficients as well as the mass factorization kernels. The SV coefficients are presented up to next-to-next-to-next-to leading order (N$^3$LO). We also use these coefficients at three loops to compute the resummed prediction for inclusive cross-section to next-to-next-to-next-to leading logarithmic accuracy (N$^3$LL) matched to next-to-next-to leading order (NNLO). We use the standard technique to derive the Mellin N-dependent coefficients and also the N-independent coefficients to achieve the resummation using the minimal prescription matching procedure. Considering the spin-2 propagator in the large extra dimensional (ADD) model, we also study the numerical impact of these three-loop SV corrections as well as the resummed predictions on the di-lepton invariant mass distribution at the 13 TeV LHC. We find that the conventional scale uncertainties in the NNLO+N$^3$LL resummed results substantially get reduced to as low as 2\% in the high invariant mass region. We also estimate the PDF uncertainties in our predictions that will be useful in the experimental searches for large extra dimensions.

==> table1.tex <==
\begin{table}[h!]
\begin{center}
{\scriptsize
%\resizebox{\linewidth}{2.25cm}{%
\resizebox{16cm}{2.50cm}{%
\begin{tabular}{ |p{1cm}|p{1.58cm}|p{1.58cm}|p{1.58cm}|p{1.58cm}|p{1.58cm}|p{1.58cm}|p{1.58cm}|p{1.58cm}| }
%\begin{tabular}{ |c|c|c|c|c|c|c|c|c| }
\hline
	\multicolumn{9}{|c|}{} \\
	\multicolumn{9}{|c|}{\small{\textbf{Gravity $gg+q\bar{q}$ subprocess at 3rd order}}} \\
	\multicolumn{9}{|c|}{} \\
\hline
{} & {} & {} & {} & {} & {} & {} & {} & \\
Q (GeV) & $(+)\mathcal{D}_{0}$  & $(-)\mathcal{D}_{1}$ & $(-)\mathcal{D}_{2}$ & $(-)\mathcal{D}_{3}$ & $(+)\mathcal{D}_{4}$ & $(+)\mathcal{D}_{5}$ & $(-)\sum\mathcal{D}_{i}$ & $(+)\delta$\\
{} & {} & {} & {} & {} & {} & {} & {} & \\
\hline
\hline
{} & {} & {} & {} & {} & {} & {} & {} & \\
$100$ & $0.1964\times~10^{-9}$ & $0.5820\times~10^{-9}$ & $0.2097\times~10^{-8}$ & $0.2247\times~10^{-8}$ & $0.7630\times~10^{-9}$ & $0.3560\times~10^{-8}$ &     $0.4073\times~10^{-9}$ & $0.3689\times~10^{-9}$ \\
%{} & {} & {} & {} & {} & {} & {} & {} & \\
\hline
{} & {} & {} & {} & {} & {} & {} & {} & \\
$1000$ & $0.7962\times~10^{-7}$ & $0.2897\times~10^{-6}$ & $0.1118\times~10^{-5}$ & $0.1233\times~10^{-5}$ & $0.4318\times~10^{-6}$ & $0.2002\times~10^{-5}$ &     $0.1265\times~10^{-6}$ & $0.9321\times~10^{-7}$ \\
\hline
{} & {} & {} & {} & {} & {} & {} & {} & \\
$2000$ & $0.1700\times~10^{-6}$ & $0.7038\times~10^{-6}$ & $0.2780\times~10^{-5}$ & $0.3091\times~10^{-5}$ & $0.1127\times~10^{-5}$ & $0.5106\times~10^{-5}$ &     $0.1705\times~10^{-6}$ & $0.1738\times~10^{-6}$ \\  
\hline
{} & {} & {} & {} & {} & {} & {} & {} & \\
$3000$ & $0.1828\times~10^{-6}$ & $0.8543\times~10^{-6}$ & $0.3429\times~10^{-5}$ & $0.3827\times~10^{-5}$ & $0.1462\times~10^{-5}$ & $0.6431\times~10^{-5}$ &     $0.3427\times~10^{-7}$ & $0.1730\times~10^{-6}$ \\  
\hline
\end{tabular}
}
\caption{\mk{Contribution of the larger logarithms and the constant term $\delta(1-z)$ at the third order in QCD for the di-lepton
production in the ADD model for different invariant masses of the di-lepton at the LHC.}}
\label{table1}
}
\end{center}
\end{table}
%\mk{Rather, can we present the results in terms of the ratios w.r.t. Leading Log i.e D0/D5, D1/D5, D2/D5, D3/D5, D4/D5 and Sum/D5, and delta/D5.}


==> table2.tex <==
\begin{table}
%\centering
\begin{center}
{\scriptsize
%\begin{tabular}{ |p{1.5cm}|p{2.0cm}|p{2.0cm}|p{2.0cm}|p{2.0cm}| }
\resizebox{12cm}{7.5cm}{%
\begin{tabular}{ |p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}| }
\hline
	\multicolumn{5}{|c|}{}\\
	\multicolumn{5}{|c|}{\small{\textbf{Resummation K factor for the signal}}} \\
	\multicolumn{5}{|c|}{}\\
\hline
	{} & {} & {} & {} &\\
Q(GeV) & LO+LL  & NLO+NLL & NNLO+NNLL & NNLO+N$^{3}$LL \\
%	{} & {} & {} & {} &\\
\hline
\hline
%\centering
	{} & {} & {} & {} &\\
$200$  &   $1.1304$  &   $1.3334$  &   $1.3457$  &   $1.3405$ \\
\hline
	{} & {} & {} & {} &\\
$400$  &   $1.1301$ &    $1.3672$  &   $1.3888$  &   $1.3827$ \\
\hline
	{} & {} & {} & {} &\\
$600$  &   $1.1345$  &   $1.3802$  &   $1.4030$  &   $1.3969$ \\
\hline
	{} & {} & {} & {} &\\
$800$  &   $1.1472$  &   $1.3911$  &   $1.4126$  &   $1.4044$ \\
\hline
	{} & {} & {} & {} &\\
$1000$  &   $1.1816$  &   $1.4214$  &   $1.4405$  &   $1.4277$ \\
\hline
	{} & {} & {} & {} &\\
$1200$  &   $1.2546$  &   $1.4927$  &   $1.5100$  &   $1.4871$ \\
\hline
	{} & {} & {} & {} &\\
$1400$  &   $1.3555$  &   $1.5926$  &   $1.6113$  &   $1.5750$ \\
\hline
	{} & {} & {} & {} &\\
$1600$  &   $1.4417$  &   $1.6701$  &   $1.6955$  &   $1.6485$ \\
\hline
	{} & {} & {} & {} &\\
$1800$  &   $1.4962$  &   $1.7077$  &   $1.7419$  &   $1.6905$ \\
\hline
	{} & {} & {} & {} &\\
$2000$  &   $1.5279$  &   $1.7176$  &   $1.7630$  &   $1.7085$ \\
\hline
	{} & {} & {} & {} &\\
$2200$  &   $1.5484$  &   $1.7140$  &   $1.7697$  &   $1.7149$ \\
\hline
	{} & {} & {} & {} &\\
$2400$  &   $1.5637$  &   $1.7045$  &   $1.7709$  &   $1.7173$ \\
\hline
	{} & {} & {} & {} &\\
$2600$  &   $1.5769$  &   $1.6940$  &   $1.7723$  &   $1.7187$ \\
\hline
	{} & {} & {} & {} &\\
$2800$  &   $1.5900$  &   $1.6813$  &   $1.7725$  &   $1.7209$ \\
\hline
	{} & {} & {} & {} &\\
$3000$  &   $1.6029$  &   $1.6698$  &   $1.7762$  &   $1.7252$ \\
\hline
\end{tabular}
}}
%\end{center}
\caption{\mk{Resummed K-factors for di-lepton invariant mass distribution at the LHC to various logarithmic accuracy in QCD.}}
\label{tab:table2}
\end{center}
\end{table}


==> tablepdf1.tex <==
%**********************************************************
%             PDF uncertainty for F.O 
%**********************************************************
\begin{table}[h!]
\begin{center}
\begin{tabular}{| *{4}{c|} }
       \hline	
	{} & {} & \multicolumn{4}{c|}{\% of Uncertainty} \\

    \cline{3-4}
PDF Name   &  No. of sets  &   $Q = 1000$GeV  &  $Q = 1500$GeV  & $Q = 2500$GeV  &   $Q = 3000$GeV  \\
    \hline
	MMHT$2014$     &   $51$  &  $5$  &  $6$  &  $12$  &   $14$  \\
    \hline
	CT$14$         &   $57$  &  $10$  &  $17$  & $32$  &   $38$    \\
    \hline
ABMP$16$               &   $30$  &  $2$  &  $6$  &  $12$  &   $13$    \\
    \hline
NNPDF$31$              &   $101$ &  $5$  &  $5$  & $7$   &   $12$    \\
    \hline
PDF$4$LHC$15$          &   $31$  &  $5$  &  $7$  & $16$  &   $19$    \\
    \hline
\end{tabular}
    \end{center}
\caption{Intrinsic PDF uncertainties calculated from {\tt lhapdf} for different PDF choices. These
uncertainties are given for two different $Q$ values of $2500$ GeV and $3000$ GeV.}
\label{tpdf1}
\end{table}

